Maximize the Foot Clearance for a Hopping Robotic Leg Considering Motor Saturation

A hopping leg, no matter in legged animals or humans, usually behaves like a spring during the periodic hopping. Hopping like a spring is efficient and without the requirement of complicated control algorithms. Position and force control are two main methods to realize such a spring-like behaviour. The position control usually consumes the torque resources to ensure the position accuracy and compensate the tracking errors. In comparison, the force control strategy is able to maintain a high elasticity. Currently, the position and force control both leads to the discount of motor saturation ratio as well as the bandwidth of the control system, and thus attenuates the performance of the actuator. To augment the performance, this letter proposes a motor saturation strategy based on the force control to maximize the output torque of the actuator and realize the continuous hopping motion with natural dynamics. The proposed strategy is able to maximize the saturation ratio of motor and thus maximize the foot clearance of the single leg. The dynamics of the two-mass model is utilized to increase the force bandwidth and the performance of the actuator. A single leg with two degrees of freedom is designed as the experiment platform. The actuator consists of a powerful electric motor, a harmonic gear and encoder. The effectiveness of this method is verified through simulations and experiments using a robotic leg actuated by powerful high reduction ratio actuators.

==> equation/kin_liftoff.tex <==
\begin{equation}
    \begin{split}
	&y_s\left(t_{lo}\right)=\left(C_{amp}+\frac{mg}{k_s}\right)  \cos{\left(\sqrt{\frac{k_s}{m}}t_{lo}+\pi\right)}+y_{s\cdot neu},\\
	&\dot y_s\left(t_{lo}\right)=\sqrt{\frac{k_s}{m}}\left(C_{amp}+\frac{mg}{k_s}\right)  \sin{\left(\sqrt{\frac{k_s}{m}}t_{lo}+\pi\right)}.
	\end{split}
	\label{eq:kin_liftoff}
\end{equation}

==> figures/exp_stiffness.tex <==
\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{3cm}
\includegraphics[width = 3.3 in]{figures/exp_stiffness.png}
\caption{Experimental results, the actual stiffness ($k_s$) of two-mass model for force control and position control in the stance phase.}
\label{fig:exp_stiffness}
\end{figure}

==> figures/structure.tex <==
\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{3cm}
\includegraphics[width  = 6.5 in]{figures/assembly_4.png}
\caption{Mechanical structure of the single leg (top). The left three subfigures are the front, side and oblique view of the single leg respectively. The right subfigure is the cross-sectional view of the hip (top) and knee joint (bottom) respectively.}
\label{fig:structure}
\end{figure*}
